Evaluating Numerical Reasoning in Text-to-Image Models

Text-to-image generative models are capable of producing high-quality images that often faithfully depict concepts described using natural language. In this work, we comprehensively evaluate a range of text-to-image models on numerical reasoning tasks of varying difficulty, and show that even the most advanced models have only rudimentary numerical skills. Specifically, their ability to correctly generate an exact number of objects in an image is limited to small numbers, it is highly dependent on the context the number term appears in, and it deteriorates quickly with each successive number. We also demonstrate that models have poor understanding of linguistic quantifiers (such as "a few" or "as many as"), the concept of zero, and struggle with more advanced concepts such as partial quantities and fractional representations. We bundle prompts, generated images and human annotations into GeckoNum, a novel benchmark for evaluation of numerical reasoning.

==> figs/autoeval_results.tex <==
\begin{wrapfigure}{r}{0.4\linewidth}
\begin{center}
\footnotesize
\begin{tikzpicture}
  \matrix(D)[matrix of nodes,nodes in empty cells,
             %row sep=-\pgflinewidth,column sep=-\pgflinewidth,
             nodes={anchor=center},
             row 1/.style={minimum height=0.8cm},
             row 2/.style={minimum height=0.8cm},
             row 3/.style={minimum height=0.8cm},
             row 4/.style={minimum height=0.8cm},
             row 5/.style={minimum height=0.8cm},
             row 6/.style={minimum height=0.8cm},
             row 7/.style={minimum height=0.8cm},
             column 1/.style={minimum width=1.1cm},
             column 2/.style={minimum width=1.1cm},
             column 3/.style={minimum width=1.1cm},
             column 4/.style={minimum width=1.1cm},
             column 5/.style={minimum width=1.1cm},
            ]
  {%
    &      &  & \\
    &      & Imagen & Muse & Dalle3 \\
    & VNLI & |[draw,fill=green!20]| \checkmark & |[draw,fill=green!20]| \checkmark & |[draw,fill=green!20]| \checkmark \\
    & TIFA & |[draw,fill=green!20]| \checkmark & |[draw,fill=blue!20]| = & |[draw,fill=blue!20]|= \\
    & CLIP & |[draw,fill=blue!20]| = & |[draw,fill=green!20]| \checkmark & |[draw,fill=blue!20]| = \\
    & Gecko & |[draw,fill=green!20]| \checkmark & |[draw,fill=blue!20]| = & |[draw,fill=blue!20]| = \\
    & DSG & |[draw,fill=red!20]| ? & |[draw,fill=red!20]| ? & |[draw,fill=red!20]| ?  \\
  };
  %\node at ($(D-1-4)!0.2!(D-2-4)$) {\scriptsize Muse};
  %\node at ($(D-4-1)!0.2!(D-4-2)$) {\scriptsize \rotatebox{90}{Imagen}};
\end{tikzpicture}
\caption{Evaluating auto-eval metrics on number generation by testing with significance level of 0.05 whether they significantly discriminate scores from correct and incorrect generations. The $\checkmark$ indicates cases where $p<0.05$ and a post-hoc comparison of average scores showed average scores for correct generations are higher than for incorrect cases.}
\end{center}
\label{fig:autoeval}
\end{wrapfigure}

==> tables/autoeval.tex <==
\begin{tabular}{c|ccccc}
\hline
          & VNLI       & TIFA       & CLIP       & Gecko      & DSG \\ \hline
Imagen 2.4 & \checkmark & \checkmark & =          & \checkmark & ?    \\
Muse 2.3   & \checkmark & =          & \checkmark & =          & ?    \\
Dalle 3    & \checkmark & =          & =          & =          & ?    \\ \hline
\end{tabular}
